On the Lack of Consensus Among Technical Debt Detection Tools

A vigorous and growing set of technical debt analysis tools have been developed in recent years -- both research tools and industrial products -- such as Structure 101, SonarQube, and DV8. Each of these tools identifies problematic files using their own definitions and measures. But to what extent do these tools agree with each other in terms of the files that they identify as problematic? If the top-ranked files reported by these tools are largely consistent, then we can be confident in using any of these tools. Otherwise, a problem of accuracy arises. In this paper, we report the results of an empirical study analyzing 10 projects using multiple tools. Our results show that: 1) these tools report very different results even for the most common measures, such as size, complexity, file cycles, and package cycles. 2) These tools also differ dramatically in terms of the set of problematic files they identify, since each implements its own definitions of "problematic". After normalizing by size, the most problematic file sets that the tools identify barely overlap. 3) Our results show that code-based measures, other than size and complexity, do not even moderately correlate with a file's change-proneness or error-proneness. In contrast, co-change-related measures performed better. Our results suggest that, to identify files with true technical debt -- those that experience excessive changes or bugs -- co-change information must be considered. Code-based measures are largely ineffective at pinpointing true debt. Finally, this study reveals the need for the community to create benchmarks and data sets to assess the accuracy of software analysis tools in terms of commonly used measures.

==> Tables/Q2-clique_summary_class.tex <==
\begin{table}[htbp]
\caption{File Cycles Reported}
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|} 
\hline
\multirow{2}{*}{Project}&DV8    &S101   &DV8    &S101  &DV8$\cap$
&               &\#sets &\#sets &\#file &\#file &S101\\ \hline

deltaspike&9&12&33&45&32\\ \hline
flume&8&11&47&47&43\\ \hline
hbase&36&39&521&272&190\\ \hline
knox&20&15&82&50&32\\ \hline
nifi&86&62&330&354&217\\ \hline
oozie&13&20&389&253&237\\ \hline
qpid-broker-j&54&40&332&514&226\\ \hline
qpid-jms&7&8&208&307&205\\ \hline
tajo&33&39&452&527&442\\ \hline
tez&17&17&136&155&113\\ \hline
\end{tabular}
\end{center}
\label{tbl:q2-file-cycles}
\end{table}


==> Tables/Q2-clique_summary_pkg.tex <==
\begin{table*}[htbp]
\caption{Package Cycles Reported}
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|} 
\hline
\multirow{2}{*}{Project}&DES &DV8 &S101 &DES &DV8 &S101 &DES $\cap$ &DES $\cap$ &DV8 $\cap$\\
&\#sets&\#sets&\#sets&\#pkg&\#pkg&\#pkg&DV8&S101&S101\\
\hline
deltaspike&2&29&9&8&34&44&7&8&34\\ \hline
flume&1&12&5&3&18&20&3&3&18\\ \hline
hbase&10&122&10&52&71&86&36&37&68\\ \hline
knox&4&32&10&7&40&50&5&4&36\\ \hline
nifi&16&145&37&41&157&164&36&34&141\\ \hline
oozie&3&76&4&28&44&45&28&27&41\\ \hline
qpid-broker-j&8&117&8&15&82&97&15&15&78\\ \hline
qpid-jms&3&23&4&12&23&29&11&12&23\\ \hline
tajo&8&77&11&37&68&75&37&37&68\\ \hline
tez&5&67&10&26&56&65&25&26&54\\ \hline
\end{tabular}
\end{center}
\label{tbl:q2-pkg-cycles}
\end{table*}


==> Tables/Q3-normed-with-history-Overlapping.tex <==
\begin{table}[htbp]
\caption{Normalized \#OverLaps with Costs $>$ Thresholds}
\footnotesize
\begin{center}
\begin{tabular}{|l|c|c|c|c|} 
\hline
Name &\#Bugs &BugChurn &\#Changes &ChangeChurn\\ \hline
DV8\_MV &2 & &1 &\\ \hline
DV8\_UI &1 & &1 &\\ \hline
\end{tabular}
\end{center}
\label{tbl:q3-norm-with-cost-overlap}
\end{table}


==> Tables/Q3-unnormed-with-history-Overlapping.tex <==
\begin{table}[htbp]
\caption{\#OverLaps with Costs $>$ Thresholds}
\begin{center}
\begin{tabular}{|l|c|c|c|c|} 
\hline
Name &\#Bugs &BugChurn &\#Changes &ChangeChurn\\ \hline
DV8\_size &3 &2 &4 &2\\ \hline
DES\_size &2 &2 &2 &1\\ \hline
S101\_size &3 &2 &3 &1\\ \hline
SCC\_size &3 &2 &4 &2\\ \hline
DES\_comp. &1 &2 &2 &1\\ \hline
SCC\_comp. &3 &2 &3 &1\\ \hline
S101\_fat &2 &2 &2 &1\\ \hline
S101\_xs &2 &2 &2 &1\\ \hline
ARCH\_fanOut & & &2 &\\ \hline
ARCH\_coCh & & &1 &\\ \hline
DV8\_issues &3 &1 &\cellcolor{lightgray}5 &1\\ \hline
DV8\_crossing &2 & &1 &\\ \hline
DV8\_MV &3 &1 &\cellcolor{lightgray}5 &\\ \hline
DV8\_UH &2 & &2 &\\ \hline
DV8\_issTypes &1 &1 &1 &1\\ \hline
SQ\_issues &2 &1 &3 &\\ \hline
\end{tabular}
\end{center}
\label{tbl:q3-with-cost-overlap}
\end{table}


==> Tables/table_tools_measures.tex <==
\begin{table}[htbp]
\caption{Measures and Tools}
\begin{center}
\begin{tabular}{|l|c|c|}
\hline
\textbf{Measure} & \textbf{Tool} & \textbf{Description}  \\ \hline
Size & \makecell{Designite \\ DV8 / SCC \\ S101} &  \makecell{Measured in LOC} \\ \hline
Complexity & \makecell{Designite \\ SCC }  & \makecell{Weighted Method Per Class} \\ \hline

Commits & \makecell{DV8 \\ JEC }  & \makecell{Commits where file is present} \\ \hline
Bug commits & \makecell{DV8 \\ JEC }  & \makecell{Bug commits where file is present} \\ \hline

Churn & \makecell{DV8 \\ JEC }  & \makecell{LOC Changed in commits} \\ \hline
Bug churn & \makecell{DV8 \\ JEC }  & \makecell{LOC Changed in bug commits} \\ \hline

Design Smells  & Designite & \makecell{Total number of Design Smells \\ among 18 varieties}  \\ \hline

Architecture Smells  & Designite & \makecell{Total number of Architecture \\ smells among 7 varieties}  \\ \hline

Clique &  DV8  & \makecell{Number of Clique \\ instances a file participates} \\ \hline
Crossing & DV8 & \makecell{Number of Crossing  \\ instances a file participates} \\ \hline

ModularityViolation & DV8 & \makecell{Number of ModularityViolation\\  instances a file participates} \\ \hline
PackageCycle & DV8 & \makecell{Number of PackageCycle \\ instances a file participates} \\ \hline
UnhealthyInheritance & DV8 & \makecell{Number of UnhealthyInheritance \\ instances a file participates} \\ \hline
UnstableInterface & DV8 & \makecell{Number of UnstableInterface \\ instances a file participates} \\ \hline

TotalFlawTypes & DV8 & \makecell{Total number of flaw types \\ a file participates}  \\ \hline
TotalFlaws & DV8 & \makecell{Total number of flaw instances \\ a file participates}  \\ \hline


CodeSmells & SonarQube & Total number of code smells  \\ \hline
Bugs & SonarQube & Total number of bugs  \\ \hline
Vulnerabilities & SonarQube & Total number of vulnerabilities  \\ \hline
SecuritySpots & SonarQube & Total number of security spots  \\ \hline
SQIssues & SonarQube & Total number of issues  \\ \hline

Fat & Structure101 & \makecell{A measure of complexity}  \\ \hline
XS & Structure101 & \makecell{A measure of excessive \\ complexity}  \\ \hline
Tangles & Structure101 & \makecell{A measure of complexity \\ caused by cyclic dependencies}  \\ \hline

%https://structure101.com/static-content/pages/resources/documents/XS-MeasurementFramework.pdf

FanIn &  Archinaut & \makecell{Number of files that depend \\ on a particular file} \\ \hline
FanOut & Archinaut & \makecell{Number of files a particular file \\ depends on} \\ \hline
TotalDeps & Archinaut & \makecell{Sum of fan in and fan out} \\ \hline
CoChangePartners & Archinaut & \makecell{Number of files a particular file \\ changed concurrently \\ within the analysis period} \\ \hline
%BugCommits & Archinaut & \makecell{Number of commits associated \\ with a bug ID this file \\ appears on} \\ \hline

\end{tabular}
\end{center}
\label{table:toolsandmetrics}
\end{table}
